Deformation Recovery: Localized Learning for Detail-Preserving Deformations

We introduce a novel data-driven approach aimed at designing high-quality shape deformations based on a coarse localized input signal. Unlike previous data-driven methods that require a global shape encoding, we observe that detail-preserving deformations can be estimated reliably without any global context in certain scenarios. Building on this intuition, we leverage Jacobians defined in a one-ring neighborhood as a coarse representation of the deformation. Using this as the input to our neural network, we apply a series of MLPs combined with feature smoothing to learn the Jacobian corresponding to the detail-preserving deformation, from which the embedding is recovered by the standard Poisson solve. Crucially, by removing the dependence on a global encoding, every \textit{point} becomes a training example, making the supervision particularly lightweight. Moreover, when trained on a class of shapes, our approach demonstrates remarkable generalization across different object categories. Equipped with this novel network, we explore three main tasks: refining an approximate shape correspondence, unsupervised deformation and mapping, and shape editing. Our code is made available at https://github.com/sentient07/LJN

==> Section/oldSection3.tex <==
\section{Approach}
 We begin by providing an overview of existing frameworks that our work builds upon.in Section~\ref{subsec:Preliminaries}. Next, we elaborate on the general framework for training and performing inference with LJN in Section~\ref{subsec:General}. In Section~\ref{subsec:supervised}, we discuss the supervised training strategy for map refinement, followed by the inference strategy that alleviates the necessity for consistent connectivity in Section~\ref{subsec:Inference}. In Section~\ref{subsec:unsupervised}, we introduce a novel technique to simultaneously learn deformation and mapping between pairs of shapes with different triangulations. Finally, in Section~\ref{subsec:ShapeEditing}, we discuss the utility of LJN for handle-based shape editing.
%
\paragraph{Notations:}
We represent shapes as compact 2-dimensional Riemannian manifolds $\mathcal{M}$ possibly with boundary $\partial \mathcal{M}$. The space of square integrable functions on $\mathcal{M}$ is noted $\mathcal{L}^{2}\left( \mathcal{M} \right)$ and equiped with the scalar product $\left< f, g \right> = \int_\mathcal{M} fg \diff \mu$. We denote the tangent plane at $p$ as $T_{p} \mathcal{M}$. We discretize $\mathcal{M}$ to be a triangle mesh $\mathcal{S} := \{\mathcal{V}, \mathcal{F}\}$ with $\mathcal{V}$  vertices and $\mathcal{F}$ faces.
On the manifold $\mathcal{M}$, the Laplace-Beltrami Operator (LBO), denoted $\Delta$ is discretized using the standard cotangent-based discretization~\cite{Pinkall1993ComputingDM}, given by $\Delta := \nabla^{T} A \nabla$, where $\nabla$ is the gradient operator and A is the area element of each face. We use a face-based discretization of the tangent plane~\cite{Azencot2013} and therefore $\nabla$ is a $\mathbf{R}^{|3\mathcal{F}|\times |\mathcal{V}|}$ matrix. Since $\Delta$ is a symmetric operator, by solving the generalized eigenvalue problem $\Delta \Psi =\lambda M \Psi$, we obtain the Laplace-Beltrami eigen-basis $\Psi=\left[\psi_1 \ldots \psi_k\right]$, where, $M$ is the diagonal-lumped vertex-mass matrix~\cite{Meyer2003}. The truncated subspace of $\mathcal{L}^{2}\left( \mathcal{M} \right)$ spanned by $\left[\psi_1 \ldots \psi_k \right]$ is a space of smooth, low-frequency functions on the manifold. Given an embedding (v.i.z vertices) $\mathcal{V}$, we consider $\bar{\mathcal{V}}$ to be its projection onto the $k$-truncated eigenbasis of the LBO. Analogously, we use $\bar{S}$ to denote the shape whose vertices are projected onto the $k$-truncated eigenspace of the LBO. 
% The gradient operator $\nabla: \mathcal{L}^{2}\left( \mathcal{M} \right) \rightarrow T_{p} \mathcal{M}$ maps functions on the manifold to tangent vector fields. Its adjoint, given as $\nabla^{T} A$, denotes the divergence operator. We use a face-based discretization of the tangent plane~\cite{Azencot2013}. Consequently, the gradient and divergence operators are $\mathbf{R}^{|3\mathcal{F}|\times |\mathcal{V}|}$ and $\mathbf{R}^{|\mathcal{V}|\times |3\mathcal{F}|}$ matrices, respectively, and $A \in \mathbf{R}^{|3\mathcal{F}|\times |3\mathcal{F}|}$ represents the area element of each face. On the manifold $\mathcal{M}$, the Laplace-Beltrami operator, denoted as $\Delta:  \mathcal{L}^{2}\left( \mathcal{M} \right) \rightarrow \mathcal{L}^{2}\left( \mathcal{M} \right)$ acts on its functional space. $\Delta$ is discretized using the standard cotangent-based discretization~\cite{Pinkall1993ComputingDM}, given by $\Delta := \nabla^{T} A \nabla$. Since $\Delta$ is a symmetric non-negative definite operator, by solving the generalized eigenvalue problem $\Delta \Psi =\lambda M \Psi$, we obtain the Laplace-Beltrami eigen-basis $\Psi=\left[\psi_1 \ldots \psi_k\right]$, where, $M$ is the diagonal-lumped vertex-mass matrix~\cite{Meyer2003}. Like a Fourier basis, these eigenfunctions, $\varphi_i$ can be sorted from low to high frequency~\cite{LevySpec} by inheriting the order of the corresponding eigenvalues. Consequently, the truncated subspace of $\mathcal{L}^{2}\left( \mathcal{M} \right)$ spanned by $\left[\psi_1 \ldots \psi_k \right]$ is a space of smooth, low-frequency functions on the manifold. Given an embedding $v: \mathcal{M} \rightarrow \mathbb{R}^3$ on the manifold, we consider the smoothed embedding $\tilde{v}^k: \mathcal{M} \rightarrow \mathbb{R}^3$ as its projection onto the $k$-truncated eigenspace of the Laplacian. Analogously, we let $\tilde{S}$ denote the shape whose vertices $\tilde{\mathcal{V}}$ are projected onto the $k$-truncated eigenspace of the Laplacian, and we called this shape \textit{spectrally projected} (see Fig.~\ref{fig:spectral_projections}). 
% Vertices of meshes are referred to as spatial embeddings or simply embeddings, whereas the eigenfunctions of the Laplacian are referred to as spectral embeddings.

% define frames
% define deformations 
For each face, we define a possibly non-orthonormal frame $\mathcal{E} := [\vec{e}_1, \vec{e}_2, \vec{N}]^T$, which is a $3 \times 3$ matrix. The frame comprises the first two edge vectors of the face, chosen by convention, and the face normal. We denote the frames for all faces collectively as $\mathbf{E} := [\mathcal{E}_1 \ldots \mathcal{E}_{|\mathcal{F}|}]$. 
% For any given point $p \in \mathbb{R}^{3} \in T_{p} \mathcal{M}$, a local deformation can be defined using a Jacobian matrix $J_{p} \in \mathbb{R}^{3 \times 3}$. Given our face-based discretization of the tangent plane, we use $J_{i} \in \mathbb{R}^{3 \times 3}$ to denote the Jacobian matrix corresponding to the $i^{th}$ face.
For any given point $x \in T_x \mathcal{M} \subseteq \mathbb{R}^{3}$, a local deformation can be defined using a Jacobian matrix $J_{x} \in \mathbb{R}^{3 \times 3}$. Given our face-based discretization of the tangent plane, Jacobians are piece-wise constant per-face. We denote $\mathbf{J} := [J_1 \ldots J_{|\mathcal{F}|}]$ to be the Jacobian across all faces represented in matrix form. 

% $x \in T \mathcal{M} \iff x \in F_i$ the $i^{th}$ face in $\mathcal{F}$, then being $J_{x}$ uniquely defined for every $x \in F_i$ we use $J_{i} \in \mathbb{R}^{3 \times 3}$ to denote the Jacobian matrix corresponding to the $i^{th}$ face.

% discretized maps
Given two discretized shapes $\mathcal{S}_1$ and $\mathcal{S}_2$ (often called source and target shapes) with respectively $n_1$ and $n_2$ vertices, we can write the map $\varphi: \mathcal{S}_1 \rightarrow \mathcal{S}_2$ between those shapes as a binary matrix $\Pi \in \mathbb{R}^{n_1 \times n_2}$ where $\Pi[{i, j}] = 1$ denotes $j^{th}$ vertex on $\mathcal{S}_2$ being the image of $i^{th}$ vertex on $\mathcal{S}_1$. When the two shapes are in 1:1 correspondence, $\Pi_{12}$ is an identity matrix.
% Note that for the pullback to the function spaces denoted by $P_{j,i}: \mathcal{L}^{2}\left(S_j\right) \rightarrow$ $\mathcal{L}^{2}\left(S_i\right)$ whose explicit form is given by $P_{j,i} = \Psi_{i}^{\dag} \Pi_{i,j} \Psi_{j}$. The rank-$k$ approximation of $P_{j,i}$,

\paragraph{Functional Map}
The functional map pipeline, introduced in \cite{ovsjanikov2012functional}, leverages an efficient and compact representation for maps between shapes. More specifically, let $\varphi: \mathcal{S}_1 \rightarrow \mathcal{S}_2$ be a pointwise map, and $\Pi_{12}$ its corresponding binary matrix. The pull-back operator associated with this map, expressed in the truncated basis and denoted as $\mathbf{C}_{21} \in \mathbb{R}^{k \times k}$, is referred to as the Functional Map~\cite{ovsjanikov2012functional}. $C_{21}: \mathcal{L}^{2}\left(S_2\right) \rightarrow \mathcal{L}^{2}\left(S_1\right)$ acts as a linear operator between the square integrable functions on the respective shapes. This can be derived from the binary matrix $\mathbf{C}_{21} = (\Psi_{1})^{\dag} \Pi_{12} \Psi_{2}$. Given the functional map $C_{21}$, in the simplest setup, we can extract back an associated $\Pi_{12}$ via a nearest-neighbors search~\cite{FMCourse}:

\begin{equation}
    (\Pi_{12})^* = \underset{\Pi_{12}}{\operatorname{argmin}} \left\|\Psi_2 C_{21}- \Pi_{12} \Psi_1\right\|_F^2
\label{eqn:FM2P2P}
\end{equation}

\paragraph{Jacobian-based deformation}
% TODO: apply a deformation ? This MUST be re-written
Let $\mathcal{S}_1, \mathcal{S}_2$ be shapes with two different vertex embeddings $\mathcal{V}_1, \mathcal{V}_2 \in \mathbb{R}^3$. We can consider the deformation between them as a per-vertex coordinate re-assignment. The linear part of this deformation quantifying the change in edge-vectors is referred to as the jacobian $\mathbf{J}_{12}$ between $\mathcal{S}_1 \rightarrow \mathcal{S}_2$. This change of edge vectors ~\cite{Sumner,BotschPoisson}) is explicitly given by:  
\begin{equation}
    \mathbf{J}_{12} = \mathbf{E}_1^{-1} \mathbf{E}_2
\label{eqn:JacClosedForm}
\end{equation}
where $\mathbf{E} = [\mathcal{E}_1 \ldots \mathcal{E}_{|F|}]$ are the frames corresponding to all faces, rewritten in matrix form. Note that while quantifying the change in edge vectors is sufficient to define $\mathbf{J}_{12}$, solving Eqn~\ref{eqn:JacClosedForm} becomes under-determined (see Chap 3.1.2 \cite{Sumner2005MeshMU}). While~\cite{Sumner} overcomes this by tetrahedralization of each face, we simply use the \emph{unit-normal} vector, as changes along normal directions are inconsequential for a surface undergoing deformation in $\mathbb{R}^3$. Given a Jacobian $\mathbf{J}_{12}$, we can compute its closest  embedding in the least-square sense by solving the following Poisson equation:
\begin{equation}
    \Delta_1 \mathcal{V}_2 = \nabla_1^{T} A_1 \mathbf{J}_{12}
\label{eqn:Poisson}
\end{equation}

% TODO: re-write... what is the goal, the story is not clear at all
Where $\nabla_1^{T} A_1$ is the divergence operator of $\mathcal{S}_1$. Since $\Delta_1$ is only semi-definite, the solution $V_2$ is not unique and is only valid up-to global translation \cite{BotschPoisson}. 
%TODO: Wow this is a sudden change 
% \cite{aigerman2022neural} proposes to learn $\mathbf{J}$ predicted by a Neural Network, but different from them, our Jacobians are $3\times3$ extrinsic matrices. 
%
\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{Figures/Method2.pdf}
  \caption{Illustration of our learning framework with spectrally projected input signal. Given a source shape and the coarse deformation signal expressed in the LBO eigen-basis, we feed in individual triangle distortion, as Jacobians, averaged to incident vertices. Then, we apply series MLPs coupled with spectral projection in the \emph{feature-space} to recover detail-preserving deformation.}
  % \Description{A woman and a girl in white dresses sit in an open car.}
  \label{fig:Method}
\end{figure}

\subsection{Detailed Deformation Learning from Coarse Signals}
\label{subsec:General}
Given a source shape \(\mathcal{S}_1\) and a coarse deformation input signal, we aim to learn the detailed deformation of the source shape, expressed as Jacobian $\mathbf{J}_{12}$. Note that our coarse input signal might not correspond to a valid shape. When these Jacobians are integrated to produce an embedding, they must correspond to a plausible shape. We let \(\mathcal{S}_2\) be the shape which the detailed Jacobian $\mathbf{J}_{12}$ corresponds to. We refer to \(\mathcal{S}_2\) as the target shape. We let $\Theta_{12} \in \mathbb{R}^{|\mathcal{V}|\times d }$ be the $d-$dimensional coarse input signal defined at vertex. Recall that, unlike ~\cite{aigerman2022neural}, we do not rely on a global encoding of the target shape but instead condition the input signal to our network using $\Theta_{12}$ alone.

 \setlength{\columnsep}{4pt}
\begin{wrapfigure}[8]{r}{0.19\textwidth}
\vspace{-0.3cm}

\begin{overpic}[width=0.19\textwidth] 
    {Figures/FeatSm2.pdf}
    \put(56.6,78.4){\footnotesize Features after}
\put(66.6,71.4){\footnotesize spectral}
   \put(63.6,64.4){\footnotesize projection}     
     \end{overpic}
     %\includegraphics[width=0.19\textwidth]{Figures/FeatSm2.pdf}
    \label{fig:Proj}
\end{wrapfigure}

 Given this input signal, we apply MLPs per-vertex in tandem with a \emph{spectral projection} layer to learn the detailed Jacobian corresponding to $\mathcal{S}_2$. The spectral projection layer projects the learned features back to the eigenbasis of the LBO operator as given in Equation~\ref{eqn:SpectralBlur}, enabling feature sharing in a small local neighborhood around each vertex. For visualization purposes, we consider a single Jacobian as a Dirac signal defined at the $i^{th}$ vertex as shown in the inset Figure (left). Then, upon projecting this signal to the eigenbasis of the LBO operator, the features are \emph{smoothly} spread out in a small neighborhood around the vertex of interest as shown in the inset Figure (right). Our learning process can then be described as follows:
\begin{equation}
    \hat{\mathbf{J}}_{12} = \mathcal{I}_{1}^{T} \mathcal{G}_{6}( \ldots (\mathrm{Proj}_{1}( \mathcal{G}_{1}(\Theta_{12} )) \ldots) 
\end{equation}

The above equation sequentially applies an MLP, $\mathcal{G} (.)$, whose specifications are provided in the Supplementary. Here, $\mathrm{Proj}(\Theta_{12}) := \Psi_1 \Psi_1^T M_1 \Theta_{12}$ expresses the features $\Theta_{12}$ in the orthonormal basis defined by $\Psi_1$. The operator $\mathcal{I}_{1}$ is a sparse row-stochastic matrix that averages quantities from faces to vertices. The non-zero entries corresponding to row $i$ of $\mathcal{I}_{1}$ sum up to 1 and are all equal to $\frac{1}{f_{i}}$, where $f_{i}$ denotes the number of faces incident on vertex $i$. Its transpose, $\mathcal{I}^{T}_{1}$ averages the per-vertex predictions back to faces. Given the ground-truth jacobian $\mathbf{J}_{12}^{*}: \mathcal{S}_1 \rightarrow \mathcal{S}_2$, to train our network, we minimize a loss function consisting of three terms as follows,

\begin{equation}
    \mathcal{L}_{\mathrm{Tr}} = \alpha_1 \left|\left| \mathbf{J}_{12}^{*}
 - \hat{\mathbf{J}}_{12}\right|\right|_F^{2} + \alpha_2 \left|\left| \mathcal{V}_2 - \hat{\mathcal{V}}_1 \right|\right|_2^{2} + \alpha_3 \left|\left| \mathbf{J}_{12}^{*}
 - \mathbf{E}_1^{-1} \mathbf{\hat{E}} \right|\right|_F^{2}
\end{equation}

Where $\hat{\mathcal{V}}_1 = \Delta_1^{-1} \nabla_1^{T} A_1 \hat{\mathbf{J}}_{12}$ is the embedding corresponding to the predicted Jacobian recovered via the Poisson solve (cf. Equation~\ref{eqn:Poisson}). The first two terms are used to supervise the positions and predicted Jacobians w.r.t the ground truth, while the third term penalizes discrepancies between the \emph{integrated} Jacobian and the ground truth Jacobian. More precisely, we compute the Jacobian corresponding to the recovered embedding $\hat{\mathcal{V}}_1$ using the corresponding non-orthonormal frame as $\mathbf{E}_1^{-1} \mathbf{\hat{E}}_1$ and minimize the discrepancy with the ground truth Jacobian. 

Our learning pipeline, along with one possible coarse input signal used in this paper, is visualized in Figure~\ref{fig:Method}. In summary, given the Jacobian between the source shape and the spectral projection of the target shape, our network is trained to reconstruct the detailed Jacobian between the source and target shapes. At inference time, the embedding can be obtained via a simple feedforward pass and a Poisson solve (cf. Eqn~\ref{eqn:Poisson}). Task-specific inference is discussed in subsequent sections.


\subsection{Supervised Learning from Spectral Inputs}
\label{subsec:supervised}
% First say the overall goal
In this section, we discuss the construction of a coarse deformation input signal geared for shape registration-related tasks. Our choice of representation for the input signal is crucial and carefully designed to be easily integrated into existing shape correspondence frameworks~\cite{ovsjanikov2012functional}.
% Construction of input signal
In order to construct the input signal, we first express the coordinate function of the target shape using the first \(k\) eigenfunctions of the LBO, referred to as the \emph{spectrally projected} shape. Let $\bar{\mathcal{S}}_2$ be the shape obtained by applying spectral projection to $\mathcal{S}_2$, and $\bar{\mathcal{V}}_2$ be its vertex set. Then, the closed-form expression for $\bar{\mathcal{V}}_2$ is given as follows:

\begin{equation}
    \mathrm{Proj}(\mathcal{V}_2) = \bar{\mathcal{V}}_2 = \Psi_2 \Psi_2^{\dag} \mathcal{V}_2 = \Psi_2 \Psi_2^T M_2 \mathcal{V}_2
\label{eqn:SpectralBlur}
\end{equation}

Where $\Psi_2^{\dag}$ is the Moore-Penrose pseudoinverse of $\Psi_2$, and  $\Psi_2^\dag = \Psi_2^T M_2$ because of orthonormality with respect to $M_2$. Denoting the frames per face corresponding to the spectrally projected shape as $\bar{\mathbf{E}}_2$, the input signal to our network is defined as follows:

\begin{equation}
\Theta_{12} := \mathcal{I}_{1} \mathbf{J}_{12} = \mathcal{I}_{1} \mathbf{E}_1^{-1} \bar{\mathbf{E}}_2
\label{eqn:JacInput}
\end{equation}
% Since shapes share same connectivity in our supervised setup, 



\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{Figures/ApproachValidation2.pdf}
  \caption{Illustration of the fidelity of our training framework. We select a \emph{seed} vertex, marked with a dotted circle. The Frobenius norm of the difference between the Jacobian at this seed vertex and all other vertices is plotted. The similarity in the distribution between the input (projected Jacobian) and the ground truth suggests the well-posed nature of our learning problem.}
  \label{fig:ApproachValidity}
  % \Description{A woman and a girl in white dresses sit in an open car.} Then, on different target shapes, we compute t
\end{figure}

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{Figures/NonIsoDefo.pdf}
%   \caption{We visualize the information lost during spectral projection for near-isometric and non-isometric deformations between two pairs of humans (first row) and animals (second row). The similarity, quantified in the annotation, represents the discrepancy between the spectral projection and the ground truth Jacobian. The similarity scores suggest that the intrinsic component does not differ significantly between near-isometric and non-isometric deformations.}
%   \label{fig:spectral_projections}
%   % \Description{A woman and a girl in white dresses sit in an open car.} Then, on different target shapes, we compute t
% \end{figure}


\paragraph{Discussion}
For a learning problem to be well-posed, distinct inputs should produce distinct outputs. We demonstrate this qualitatively on pairs of shapes, as shown in Figure~\ref{fig:ApproachValidity}. We consider a fixed source shape and a vertex of interest in this source shape as the "seed" vertex, say the $i^{th}$ vertex. We then plot the Frobenius norm of the difference between the input signal at the $i^{th}$ vertex and all the remaining vertices, expressed as $\|\Theta_{i, 12} - \Theta_{j, 12}\|_F \forall i \neq j$, in the first row. Similarly, in the second row, we plot the difference between the ground truth Jacobian $i^{th}$ vertex and all the remaining vertices, $\|J^{*}_{i, 12} - J^{*}_{j, 12}\|_F \forall i \neq j$. The similarity in the distributions of the norm at each vertex between input and ground-truth across different deformations asserts the well-posed nature of our learning problem.


\subsection{Inference: Meshes with differing connectivity.}
\label{subsec:Inference}
The requirement for shapes to be in 1-1 correspondence when constructing the input signal is impractical for real-world applications. To address this, we utilize the Functional Map framework to model deformations between shapes with differing connectivities. Therefore, given a pair of shapes $\mathcal{S}_1, \mathcal{S}_2$ with differing connectivity and a functional map $C_{21}$ between them, we aim to extract the deformation $\hat{\mathbf{J}}_{12}$ between them. The Functional Map can be estimated via an existing Deep Functional Map (DFM) framework~\cite{sun2023spatially,ULRSSM}, or alternatively, using our unsupervised method detailed in Section~\ref{subsec:unsupervised}.

Different from training time, at inference, we first write the spectral projection of the coordinate function of the target shape and `pull' back the embedding function to the source shape using the functional map, as follows,

\begin{equation}
    \bar{\mathcal{V}}_1 = \Psi_1 C_{21} \Psi_2^{\dag} \mathcal{V}_2
\label{eqn:BlurInference}
\end{equation}

The above equation expresses the coordinate function of the target shape in the LBO eigenbasis of the source shape, with the functional map acting as the change of basis operator. Since $\mathcal{V}_1$ and $\bar{\mathcal{V}}_1$ share the same connectivity, we can define the input to our network as given in Equation~\ref{eqn:JacInput} and perform a feedforward pass to obtain $\hat{\mathbf{J}}_{12}$. 
To retrieve the embedding but instead of simply solving the Poisson equation~\ref{eqn:Poisson}, we also leverage the point-wise map $\Pi_{12}$ arising from the Functional Map (using c.f Eqn~\ref{eqn:FM2P2P}). We do this in order to address numerical errors in the learned Jacobian which might lead to detailed deformation but ``un-aligning'' surface as highlighted in Figure~\ref{fig:UnAligning}. To this end, our embedding recovery from Jacobian is solved via the following minimization,

\begin{equation}
    \hat{\mathcal{V}}_1 = \underset{\hat{\mathcal{V}}_1} {\operatorname{min}} \hspace{1mm} \alpha_4 \left|\left| \hat{\mathcal{V}}_1 - \Pi_{12} \mathcal{V}_2 \right|\right|^2_{M_{1}} + \alpha_5 \left|\left| \Delta_1 \hat{\mathcal{V}}_1 - \nabla_1^{T} A_{1} \hat{\mathbf{J}}_{12} \right|\right|^2_{M_{1}} + \left|\left| \hat{\mathcal{V}}_1 \right|\right|^2_{\Delta_{1}}
\label{eqn:EmbedRecovery}
\end{equation}

Where, the first term enforces a spatial constraint to ensure that the recovered embedding remains geometrically close to the target surface, while the second term ensures that the recovered embedding respects the learned Jacobians. The final term promotes smoothness in the recovered embedding by favoring a minimum norm solution. Setting the gradient of the above expression w.r.t $\mathcal{V}_1$ to be zero yields,

\begin{equation}
    (\Delta_1 + \alpha_4 M_1 + \alpha_5 \Delta_1^T M_1 \Delta_1) \hat{\mathcal{V}}_1 = \alpha_4 M_1 \Pi_{12} \mathcal{V}_2 + \alpha_5 \Delta_1^T M_1 \nabla_1^{T} A_1 \hat{\mathbf{J}}_{12}
\label{eqn:EmbedRecoveryBacksub}
\end{equation}

Since the LHS in the above expression depends only on the Laplacian and the mass matrix, it can be pre-factored. If registration is the final goal, one can obtain a refined pointwise-map using the deformed embedding $\hat{\mathcal{V}}_1$. This can be done by the following minimization, 

\begin{equation}
    \Pi_{12}^{*} = \underset{\Pi^*_{12}}{\operatorname{argmin}} \| \hat{\mathcal{V}}_1 - \Pi^*_{12} \mathcal{V}_2 \|^2_2
\label{eqn:FinalP2P}
\end{equation}

which yields, $\Pi_{12}^{*} = \mathrm{NNSearch}(\hat{\mathcal{V}}_1, \mathcal{V}_2)$.

\subsection{Unsupervised Deformation Learning and Mapping}
\label{subsec:unsupervised}

% Conditioning the input signal to be the Jacobian corresponding to deformation expressed in a reduced basis facilitates a robust training framework. However, our supervised method cannot generalize to all plausible deformations. Therefore, 
In this section, we propose an unsupervised training methodology on a collection of shapes without consistent triangulation, leveraging the Functional Map framework. Unlike in Section~\ref{subsec:Inference}, we do not assume to have access $C_{21}$ to as input, but rather \emph{learn} it alongside $\mathbf{J}_{12}$. To this end, we employ the two-branch Deep Functional Map (DFM)~\cite{sun2023spatially,ULRSSM}, a de-facto standard for non-rigid shape matching—and combine it with LJN. We denote the feature extractor within the standard DFM~\cite{DFN} corresponding to source and target shapes as $\mathcal{D}_1$ and $\mathcal{D}_2$ respectively. Between the input pair, we estimate the Functional Map in a differentiable manner, similar to ~\cite{ULRSSM} as follows,
\begin{equation}
    \hat{C}_{21} = \Psi_{1}^{\dag} \tilde{\Pi}_{12} \Psi_{2}
\label{eqn:SoftFmap}
\end{equation}
Where $\tilde{\Pi}_{12} = \operatorname{Softmax}\left(\mathcal{D}_{1} \mathcal{D}_{2}^T / \tau\right)$, is the soft pointwise map with $\tau=0.07$ being the temperature parameter. Using the $\hat{C}_{21}$ estimated above, we compute $\bar{\mathcal{V}}_1$ using Eqn~\ref{eqn:BlurInference} and use it to compute $\Theta_{12}$ via Eqn~\ref{eqn:JacInput}. Then, we perform a feed-forward pass through LJN to get predicted Jacobian $\hat{\mathbf{J}}_{12}$. We train the two-branch functional map network and our LJN jointly by minimizing the following loss.

\begin{equation}
    \mathcal{L}_{\mathrm{un}} = \sum_{i\in\{1,2\}, j\in\{2,1\}} \left\|\mathbf{C}_{i,j}^T \mathbf{C}_{i,j}-\mathbf{I}\right\|_F^2+\left\|\mathbf{C}_{i,j}-\hat{\mathbf{C}}_{i,j}\right\|_F^2 + \mathcal{L}_{\mathrm{J}} (\mathbf{J}_{j,i})
\label{eqn:UnsupFMLoss}
\end{equation}

Where, $C_{i,j}$ is the predicted Functional Map and $\hat{C}_{i,j}$ is the functional map arising from the soft-pointwise map (c.f Eqn~\ref{eqn:SoftFmap}). Note that the summation in the above equation optimizes the Functional Map and Jacobian in both directions. For simplicity and consistency, we elaborate on the minimization objective for $\mathbf{J}_{1,2}$ while noting that the same applies analogously to $\mathbf{J}_{2,1}$. Our unsupervised deformation objective $\mathcal{L}_{\mathrm{J}} (\mathbf{J}_{1,2})$ is given as follows,

\begin{equation}
    \mathcal{L}_{\mathrm{J}} (\hat{\mathbf{J}}_{12}) = \left\| \mathring{\mathbf{J}}_{12} - \hat{\mathbf{J}}_{12}\right\|^2_F + \alpha_6 \left\|\hat{\mathbf{J}}_{12} - \mathcal{H}_{1} \hat{\mathbf{J}}_{12}\right\|_F^2 + \alpha_7 \left\| \mathrm{det}(\hat{\mathbf{J}}_{12}) - 1. \right\|^2
\label{eqn:UnsupLoss}
\end{equation}

Where,  $\mathring{\mathbf{J}}_{12}$ is the Jacobian corresponding to the deformation prescribed by $\tilde{\Pi}_{12}$. More specifically, we first compute the deformation of the source embedding as $\mathring{\mathcal{V}_1} = \tilde{\Pi}_{12}\mathcal{V}_2$. Then, denoting the frame corresponding to mesh $\mathring{\mathcal{S}}_1 = \{\mathring{\mathcal{V}_1}, \mathcal{F}_1\}$ as $\mathring{\mathbf{E}}_1$, we define $\mathring{\mathbf{J}}_{12} := \mathbf{E}^{-1}_1 \mathring{\mathbf{E}}_1$. The second term in the loss function is a smoothness prior, enforcing minimal norm differences between predicted Jacobians corresponding to adjacent faces with $\mathcal{H}_{1}$ denoting the unsigned face-face incidence matrix. The third term promotes volume preservation, an important regularization term, which is deemed empirically useful when supervising with $\tilde{\Pi}_{12}$ due to the effect of truncation of basis.

\subsection{Interactive Editing}
\label{subsec:ShapeEditing}
To demonstrate that the LJN deformation framework is applicable to tasks beyond shape correspondence, we consider the task of interactive shape editing. In this scenario, a user prescribes deformation at selected vertices (handles). Our goal is to produce a minimal distortion embedding consistent with the user-prescribed deformation. Interactive editing can often result in meshes with degenerate elements, making the computation of differential operators and their eigendecomposition ill-defined. Therefore, we use the closest rotation matrix to the ground truth Jacobians as our input signal. This scenario is more challenging since the input deformation signal does not correspond to a valid shape, i.e, there is no guarantee that an embedding exists whose differentials correspond to the input signal.  
To compute the input signal, we apply polar decomposition to the ground truth Jacobian $\mathbf{J}^{*}_{12} = \mathcal{Q}_{12} \mathcal{W}_{12}$, where $\mathcal{Q}_{12}$ is the orthonormal matrix and $\mathcal{W}_{12}$ is an SPD matrix. Since our training pairs consist of valid shapes, $\mathbf{J}^{*}_{12}$ is always full rank and admits a unique polar decomposition. Therefore, to compute $\Theta_{12}$ (cf. Eqn~\ref{eqn:JacInput}), we use $\mathcal{Q}_{12}$ instead of $\mathbf{E}_1^{-1}\bar{\mathbf{E}}_2$. The rest of the training pipeline remains identical to our discussions in Section~\ref{subsec:supervised}. In summary, given rotation matrices averaged over the one-ring neighborhood, we learn the Jacobian corresponding to the detail-preserving deformation.
